Phrase-BERT: Improved Phrase Embeddings from BERT with an Application to Corpus Exploration

Phrase representations derived from BERT often do not exhibit complex phrasal compositionality, as the model relies instead on lexical similarity to determine semantic relatedness. In this paper, we propose a contrastive fine-tuning objective that enables BERT to produce more powerful phrase embeddings. Our approach (Phrase-BERT) relies on a dataset of diverse phrasal paraphrases, which is automatically generated using a paraphrase generation model, as well as a large-scale dataset of phrases in context mined from the Books3 corpus. Phrase-BERT outperforms baselines across a variety of phrase-level similarity tasks, while also demonstrating increased lexical diversity between nearest neighbors in the vector space. Finally, as a case study, we show that Phrase-BERT embeddings can be easily integrated with a simple autoencoder to build a phrase-based neural topic model that interprets topics as mixtures of words and phrases by performing a nearest neighbor search in the embedding space. Crowdsourced evaluations demonstrate that this phrase-based topic model produces more coherent and meaningful topics than baseline word and phrase-level topic models, further validating the utility of Phrase-BERT.

==> sections/6-experiment.tex <==
\section{Experiment Details}
\micomment{merge this into the previous section}



\paragraph{Dataset for phrase semantics evaluation} Please refer to Table \ref{tab:dataset} for details.

\paragraph{Dataset for lexical evaluation} 
In order not to give an unfair advantage to our model \name, which has seen phrases extracted from wikipedia , we turn to another domain from which we extract the vocabularies for the nearest neighbour diversity experiments. We leverage on a large corpus from \cite{storium2020}, which contains 125M tokens of narrative texts from more than 50 categories. We select vocabulary by including both unigrams and phrases.
First, we include 50k word types detected by spaCy's English tokenizer~\citep{spacy} that occur more than five times in the corpus. We augment this vocabulary with phrases by extracting constituent chunks from the output of a constituency parser.\footnote{We use the fast Stanford shift-reduce parser from~\citet{corenlp}.} Specifically, we extract all verb, noun, adjective, and adverb phrases from the data, and add the most frequent 75K phrases into our vocabulary set.

\paragraph{Phrase Representations} Except for GloVe and spanBERT, we use the mean-pooled representation over the last layer outputs from all models as phrase representations. This follows from \citet{yu2020assessing}, which tests a variety of phrase representations, including the mean-pooled embedding, the first-token embedding (the \textbf{CLS}-vector), the head-token embedding and others, and find that the mean-pooled embedding consistently outperforms or is comparable with other representation type for phrases, both in setting with and without task-specific fine-tuning. Similarly for sentences, mean-pooling over the last layer output also outperforms other representations in semantics evaluation tasks \cite{reimers-2019-sentence-bert, conneau2018-sent-eval}. 
For GloVe, we perform mean-pooling over all component vectors.
For spanBERT, 



==> sections/deleted-5-phrase-div-eval.tex <==



==> sections/deleted-7-result.tex <==
\section{Results}





==> tables/dataset-stats-back.tex <==
\begin{table}
	\begin{center}
		\small
    \begin{adjustbox}{max width=\textwidth}
		\begin{tabular}{ p{1cm}p{6cm}}
            % column names
			\toprule
			\textbf{Dataset} & \textbf{Example} \\
			\midrule
			
			% dataset
			Turney
			& 
			% example
			(learned person, pundit, ``match'') \\
			\midrule
			
			
			% dataset
			BiRD
			& 
			% example
			(business development, economic growth, $0.586$) \\
			\midrule

			% dataset
            PPDB-filtered
			& 
			% example
			(global \textcolor{red}{affairs}, world \textcolor{red}{affairs}, ``positive'') \newline
			(world \textcolor{red}{affairs}, domestic \textcolor{red}{affairs}, ``negative'') \\
			\midrule

			% dataset
            PPDB
			& 
			% example
			(actively participate, play an activate role, ``positive")\\
			\midrule

			% dataset
            PAWS-short
			& 			
			% example
			(a \textcolor{red}{variable} version of the \textcolor{red}{basic} lyrics, \newline
			a \textcolor{red}{basic} version of the \textcolor{red}{variable} lyrics, ``negative") \\
			\bottomrule
	
		\end{tabular}
    \end{adjustbox}
	\end{center}
	\caption{Datasets and examples used in our phrase embedding evaluation.}
	\label{tab:dataset}
\end{table}


